StablePose: Learning 6D Object Poses from Geometrically Stable Patches

We introduce the concept of geometric stability to the problem of 6D object pose estimation and propose to learn pose inference based on geometrically stable patches extracted from observed 3D point clouds. According to the theory of geometric stability analysis, a minimal set of three planar/cylindrical patches are geometrically stable and determine the full 6DoFs of the object pose. We train a deep neural network to regress 6D object pose based on geometrically stable patch groups via learning both intra-patch geometric features and inter-patch contextual features. A subnetwork is jointly trained to predict per-patch poses. This auxiliary task is a relaxation of the group pose prediction: A single patch cannot determine the full 6DoFs but is able to improve pose accuracy in its corresponding DoFs. Working with patch groups makes our method generalize well for random occlusion and unseen instances. The method is easily amenable to resolve symmetry ambiguities. Our method achieves the state-of-the-art results on public benchmarks compared not only to depth-only but also to RGBD methods. It also performs well in category-level pose estimation.

==> figures/more_visual_results.tex <==
%!TEX root = ../sceneparse.tex

\begin{figure*}[!h] \centering
    \vspace{-4pt}
	\begin{overpic}[width=1.0\linewidth,tics=5]{figures/images/more_visual_results}%,grid
    %\put(0.4,37){\small \rule[-0.4ex]{0.2ex}{1.0em}\rule[0.5ex]{35.5ex}{0.1em} \tless \rule[0.5ex]{35.5ex}{0.1em}\rule[-0.4ex]{0.2ex}{1.0em}}
    %\put(67.7,37){\small \rule[-0.4ex]{0.2ex}{1.0em}\rule[0.5ex]{12.7ex}{0.1em} \lmo \rule[0.5ex]{12.7ex}{0.1em}\rule[-0.4ex]{0.2ex}{1.0em}}
    \end{overpic}\vspace{-8pt}
   \caption{More visual results of 6D object pose estimation by StablePose on \tless, \lmo, \nocs and \snp.
   }
   \label{fig:more_visual_results}
\end{figure*} 

==> figures/object_evaluation.tex <==
%!TEX root = ../sceneparse.tex

\begin{figure}[t!] \centering\vspace{-4pt}
	\begin{overpic}[width=1.0\linewidth,tics=5]{figures/images/object_evaluation}
    \end{overpic}\vspace{-8pt}
   \caption{
   Quantitative results of StablePose for individual objects in \tless. The performance is evaluated by \evsd (VIVO). The red, green and blue blocks correspond to high (0.8-1), middle (0.6-0.8) and low (0-0.6) \evsd (VIVO) values, respectively.
   }
   \label{fig:object_evaluation}
\end{figure} 

==> figures/visual_ablation.tex <==
%!TEX root = ../sceneparse.tex

\begin{figure*}[t!] \centering\vspace{-4pt}
	\begin{overpic}[width=1.0\linewidth,tics=5]{figures/images/visual_ablation}%,grid
    \put(-1.5,2){\rotatebox{90}{\small StablePose}}
    \put(-1.5,14.5){\rotatebox{90}{\small Baseline}}
    \put(-1.5,28){\rotatebox{90}{\small Scene}}
    %\put(0.4,37){\small \rule[-0.4ex]{0.2ex}{1.0em}\rule[0.5ex]{35.5ex}{0.1em} \tless \rule[0.5ex]{35.5ex}{0.1em}\rule[-0.4ex]{0.2ex}{1.0em}}
    %\put(67.7,37){\small \rule[-0.4ex]{0.2ex}{1.0em}\rule[0.5ex]{12.7ex}{0.1em} \lmo \rule[0.5ex]{12.7ex}{0.1em}\rule[-0.4ex]{0.2ex}{1.0em}}
    \end{overpic}\vspace{-8pt}
   \caption{Visual results of 6D object pose estimation by \emph{without patch-wise pose estimation} baseline and StablePose on \tless.
   }
   \label{fig:visual_ablation}
\end{figure*} 
\vspace{12pt} 

==> sec/ablation.tex <==
%!TEX root = sceneparse.tex



\section{Visual Ablation of Patch-wise Pose Estimation}
\label{sec:ablation}
To further illustrate the effect of the patch-wise pose estimation component, we qualitatively compare StablePose with \emph{without patch-wise pose estimation} baseline on \tless in \Fig{visual_ablation}.
It shows that StablePose produces more accurate results on most shown cases, which demonstrates patch-wise pose estimation indeed provides substantial enhancements for improving object pose accuracy.

\input{figures/visual_ablation}


==> sec/augmentation.tex <==
%!TEX root = sceneparse.tex

\section{Data Augmentation of Depth Images}
0.5h

occlusion

==> sec/nocs.tex <==
%!TEX root = sceneparse.tex


\section{Quantitative Comparison on \nocs}
\label{sec:nocs}
We compare StablePose with two baselines on \nocs. The baselines are~NOCS~\cite{wang2019normalized} and 6-pack~\cite{wang20206}. Note that while StablePose and NOCS take single RGBD images as input, 6-pack process RGBD videos and estimate the object poses of all frames jointly, which could greatly boost the pose estimation performance.
We use the following evaluation metrics proposed in~\cite{wang2019normalized,wang20206}: $5^{\circ}5cm$, $IoU25$, $R_{err}$ and $T_{err}$.
In \Cref{tab:nocs}, we report the quantitative results.
It shows that StablePose beats all these baselines in two metrics ($5^{\circ}5cm$, $T_{err}$) and achieves comparable performances in the others ($IoU25$, $R_{err}$).
This demonstrates the cross-instance generality of StablePose. It also reveals that the generality of category-level pose estimation relies more on geometry instead of appearance.

\begin{table}
\footnotesize\centering
\caption{
Quantitative comparison on \nocs.
}\vspace{-6pt}
\label{tab:nocs}
\begin{tabular}{ccccc}
\toprule
  & Metric & NOCS~\cite{wang2019normalized} & 6-pack~\cite{wang20206} & StablePose \\ \midrule
\multirow{4}{*}{Bottle} & $5^{\circ}5cm$ & 5.5 & 24.5 & \textbf{37.0}  \\
 & $IoU25$ & 48.7 & 91.1 & \textbf{94.8}  \\
 & $R_{err}$ & 25.6 & \textbf{15.6} & 19.4 \\
 & $T_{err}$ & 14.4 & \textbf{4.0} & 4.5 \\ \midrule
\multirow{4}{*}{Bowl} & $5^{\circ}5cm$ & 62.2 & 55.0 & \textbf{76.6}  \\
 & $IoU25$ & 99.6 & \textbf{100.0} & \textbf{100.0}  \\
 & $R_{err}$ & 4.7 & 5.2 & \textbf{4.0} \\
 & $T_{err}$ & 1.2 & 1.7 & \textbf{1.1} \\ \midrule
\multirow{4}{*}{Camera} & $5^{\circ}5cm$ & 0.6 & \textbf{10.1} & 4.3  \\
 & $IoU25$ & \textbf{90.6} & 87.6 & 85.5  \\
 & $R_{err}$ & \textbf{33.8} & 35.7 & 43.9 \\
 & $T_{err}$ & \textbf{3.1} & 5.6 & 4.5 \\ \midrule
\multirow{4}{*}{Can} & $5^{\circ}5cm$ & 7.1 & \textbf{22.6} & 17.2  \\
 & $IoU25$ & 77.0 & \textbf{92.6} & 90.5  \\
 & $R_{err}$ & 16.9 & \textbf{13.9} & 20.5 \\
 & $T_{err}$ & \textbf{4.0} & 4.8 & 4.4 \\ \midrule
\multirow{4}{*}{Laptop} & $5^{\circ}5cm$ & 25.5 & 63.5 & \textbf{80.0}  \\
 & $IoU25$ & 94.7 & 98.1 & \textbf{99.4}  \\
 & $R_{err}$ & 8.6 & \textbf{4.7} & 4.8 \\
 & $T_{err}$ & 2.4 & 2.5 & \textbf{2.1} \\ \midrule
\multirow{4}{*}{Mug} & $5^{\circ}5cm$ & 0.9 & \textbf{24.1} & 17.7  \\
 & $IoU25$ & 82.8 & \textbf{95.2} & 92.9  \\
 & $R_{err}$ & 31.5 & 21.3 & \textbf{19.8} \\
 & $T_{err}$ & 4.0 & \textbf{2.3} & 3.8 \\ \midrule
\multirow{4}{*}{Overall} & $5^{\circ}5cm$ & 17.0 & 33.3 & \textbf{38.8}  \\
 & $IoU25$ & 82.2 & \textbf{94.2} & 93.9  \\
 & $R_{err}$ & 20.2 & \textbf{16.0} & 18.7 \\
 & $T_{err}$ & 4.9 & 3.5 & \textbf{3.4} \\
\bottomrule
\end{tabular}
\vspace{1em}\vspace{-16pt}
\end{table} 

==> sec/object.tex <==
%!TEX root = sceneparse.tex

%\newcommand{\evsd}{$e_{VSD}$\xspace}


\section{Quantitative Evaluation of Individual Objects}
\label{sec:object}
To further illustrate the strengths and weaknesses of StablePose on different object types, we provide the quantitative results of individual objects of \tless in \Fig{object_evaluation}. The number above each object is the \evsd (VIVO) value of the corresponding object. The red, green and blue blocks represent high (0.8-1), middle (0.6-0.8) and low (0-0.6) \evsd (VIVO) values, respectively.
The results show that StablePose works the best on objects with sufficient number of large planar and/or cylindrical patches.
This verifies the effects of our network designs that utilize planar and/or cylindrical patches.
The inferior results of composite objects with multiple parts and objects with concave geometry are due to the incapability of extracting repeatable patches from the noisy depth images by the current patch extraction approach.

\input{figures/object_evaluation}


==> sec/shapenetpose.tex <==
%!TEX root = sceneparse.tex

\section{The ShapeNetPose dataset}
\label{sec:shapenetpose}

\subsection{Overview}
\snp consists of rendered RGBD images of objects from 22 categories. For each category, 80\% and 20\% objects are selected for training and testing respectively. All the objects are normalized into a $1m\times1m\times1m$ box. Each selected object is rendered from a random view-point to generate a RGBD image. Random occlusions are added to each RGBD image.
Statistics of \snp is listed in \Cref{tab:snp}.


\subsection{Evaluation Metrics}
The results on \snp are evaluated by four evaluation metrics: $10^{\circ}10cm$, $IoU25$, $R_{err}$ and $T_{err}$ as proposed in~\cite{wang2019normalized,wang20206}. Note that, as \snp is a synthetic dataset, to facilitate the evaluation, all the objects in \snp are normalized into a $1m\times1m\times1m$ cube.


\begin{table}
\footnotesize\centering
\caption{
Statistics of \snp.
}\vspace{-6pt}
\label{tab:snp}
\begin{tabular}{ccc}
\toprule
Category  & \#Train object & \#Test object \\ \midrule
airplane & 500 & 100  \\
ashcan & 200 & 40  \\
bag & 50 & 10 \\
bathtub & 500 & 100 \\
bed & 100 & 20 \\
bench & 500 & 100  \\
bottle & 400 & 80  \\
bus & 500 & 100 \\
camera & 80 & 16 \\
can & 80 & 16 \\
car & 500 & 100 \\
chair & 500 & 100  \\
display & 500 & 100  \\
earphone & 50 & 10   \\
guitar & 500 & 100 \\
helmet & 100 & 20 \\
%jar & 500 & 96 \\
lamp & 500 & 100  \\
laptop & 300 & 60 \\
pot & 500 & 100  \\
skateboard & 100 & 20   \\
sofa & 500 & 100   \\
table & 500 & 100 \\
\bottomrule
\end{tabular}
\vspace{1em}\vspace{-16pt}
\end{table}

==> sec/stability_long.tex <==
%!TEX root = sceneparse.tex

\section{Stability Analysis for Pose Estimation}
\label{sec:review}

\input{figures/stability}

We describe stability analysis of 3D shapes, also known as slippage analysis, and investigate its relation to object pose estimation. Formally, the geometric stability of a 3D shape can be characterized by the rigid transformations (translation and/or rotation) that minimizes point-to-plane error metric.
Intuitively, if a 3D shape is transformed by a rigid transformation without introducing significant motion along the normal direction at each surface point, it is called geometrically unstable (or slippable) along that transformation. If there is no such transformation, the shape is stable. See Figure~\ref{fig:stability}(a-d) for a few examples with different stability.

\input{figures/overview}

\paragraph{Stability analysis}
Mathematically, given a 3D point set $\mathcal{P}=\{\bv_i, \bn_i\}$ sampled on the template model surface, we want to find a rigid transformation $[\bR|\bt]$ which minimizes the following point-to-plane error at all points:
%
\begin{equation}\label{eq:alignerror}
\min_{[\bR,\bt]}\sum_{i}{[(\bR\bv_i+\bt)\cdot \mathbf{n}_i]^2},
\end{equation}
where $\bR$ and $\bt$ are rotation and translation, respectively.

The rotation $\bR$ is nonlinear but can be linearized assuming infinitesimal rotations:
\begin{equation}\label{eq:rotlinear}
\mathbf{R} \approx \begin{pmatrix}
                     1 & -\gamma & \beta \\
                     \gamma & 1 & -\alpha \\
                     -\beta & \alpha & 1 \\
                   \end{pmatrix},
\end{equation}
for Euler angles $\alpha$, $\beta$, and $\gamma$ around the X, Y, and Z axes, respectively.
This reduces the rotation of $\bv_i \in \mathbf{V}$ by $\bR$ into a
displacement of it by a vector $[\br \times \bv_i + \bt]$, where
$\br=(\alpha, \beta, \gamma)$. Substituting this into Equation (\ref{eq:alignerror}),
we therefore aim to find a 6-vector $[\br^T, \bt^T]$ that minimizes
\begin{equation}\label{eq:linearerror}
\min_{[\br,\bt]}\sum_{i}{[\bv_i \cdot \bn_i + \br \cdot (\bv_i \times \bn_i) + \bt \cdot \bn_i]}.
\end{equation}
%We minimize $\mathcal{E}$ with respect to $\alpha$, $\beta$, $\gamma$, $\mathbf{t}_x$, $\mathbf{t}_y$, and $\mathbf{t}_z$ by setting their partial derivatives to zero:
%\begin{equation}\label{eq:derivatives}
%\begin{aligned}
%\frac{\partial \mathcal{E}}{\partial \alpha}= \sum_{i}2c_{i,x}[\mathbf{p}_i \cdot \mathbf{n}_i + \mathbf{r} \cdot (\mathbf{p}_i \times \mathbf{n}_i) + \mathbf{t} \cdot \mathbf{n}_i]=0\\
%\frac{\partial \mathcal{E}}{\partial \beta}= \sum_{i}2c_{i,y}[\mathbf{p}_i \cdot \mathbf{n}_i + \mathbf{r} \cdot (\mathbf{p}_i \times \mathbf{n}_i) + \mathbf{t} \cdot \mathbf{n}_i]=0\\
%\frac{\partial \mathcal{E}}{\partial \gamma}= \sum_{i}2c_{i,z}[\mathbf{p}_i \cdot \mathbf{n}_i + \mathbf{r} \cdot (\mathbf{p}_i \times \mathbf{n}_i) + \mathbf{t} \cdot \mathbf{n}_i]=0\\
%\frac{\partial \mathcal{E}}{\partial t_x}= \sum_{i}2n_{i,x}[\mathbf{p}_i \cdot \mathbf{n}_i + \mathbf{r} \cdot (\mathbf{p}_i \times \mathbf{n}_i) + \mathbf{t} \cdot \mathbf{n}_i]=0\\
%\frac{\partial \mathcal{E}}{\partial t_y}= \sum_{i}2n_{i,y}[\mathbf{p}_i \cdot \mathbf{n}_i + \mathbf{r} \cdot (\mathbf{p}_i \times \mathbf{n}_i) + \mathbf{t} \cdot \mathbf{n}_i]=0\\
%\frac{\partial \mathcal{E}}{\partial t_z}= \sum_{i}2n_{i,z}[\mathbf{p}_i \cdot \mathbf{n}_i + \mathbf{r} \cdot (\mathbf{p}_i \times \mathbf{n}_i) + \mathbf{t} \cdot \mathbf{n}_i]=0\\
%\end{aligned}
%\end{equation}
%
This is a linear least-squares problem which amounts to solve a linear system $C\mathbf{x}=0$ with $\mathbf{x}=[\br^T, \bt^T]$. $C$ is a $6\times 6$ covariance matrix of the rigid transformation accumulated over all sample points:
\begin{equation}\label{eq:covariance}
C=\sum_{i}\left[
             \begin{array}{cccccc}
             \mathbf{u}_{ix} \\ \mathbf{u}_{iy} \\ \mathbf{u}_{iz} \\ \mathbf{n}_{ix} \\ \mathbf{n}_{iy} \\ \mathbf{n}_{iz} \\
             \end{array}
\right]
\left[
             \begin{array}{c}
             \mathbf{u}_{ix} \ \mathbf{u}_{iy} \  \mathbf{u}_{iz} \  \mathbf{n}_{ix} \  \mathbf{n}_{iy} \  \mathbf{n}_{iz} \\
             \end{array}
\right],
\end{equation}
%\begin{equation}\label{eq:covariance}
%\sum_{i}\left[
%             \begin{array}{cccccc}
%             \mathbf{c}_{ix}\mathbf{c}_{ix} & \mathbf{c}_{ix}\mathbf{c}_{iy} & \mathbf{c}_{ix}\mathbf{c}_{iz} & \mathbf{c}_{ix}\mathbf{n}_{ix} & \mathbf{c}_{ix}\mathbf{n}_{iy} & \mathbf{c}_{ix}\mathbf{n}_{iz} \\
%             \mathbf{c}_{iy}\mathbf{c}_{ix} & \mathbf{c}_{iy}\mathbf{c}_{iy} & \mathbf{c}_{iy}\mathbf{c}_{iz} & \mathbf{c}_{iy}\mathbf{n}_{ix} & \mathbf{c}_{iy}\mathbf{n}_{iy} & \mathbf{c}_{iy}\mathbf{n}_{iz}\\
%             \mathbf{c}_{iz}\mathbf{c}_{ix} & \mathbf{c}_{iz}\mathbf{c}_{iy} & \mathbf{c}_{iz}\mathbf{c}_{iz} & \mathbf{c}_{iz}\mathbf{n}_{ix} & \mathbf{c}_{iz}\mathbf{n}_{iy} & \mathbf{c}_{iz}\mathbf{n}_{iz}\\
%             \mathbf{n}_{ix}\mathbf{c}_{ix} & \mathbf{n}_{ix}\mathbf{c}_{iy} & \mathbf{n}_{ix}\mathbf{c}_{iz} & \mathbf{n}_{ix}\mathbf{n}_{ix} & \mathbf{n}_{ix}\mathbf{n}_{iy} & \mathbf{n}_{ix}\mathbf{n}_{iz}\\
%             \mathbf{n}_{iy}\mathbf{c}_{ix} & \mathbf{n}_{iy}\mathbf{c}_{iy} & \mathbf{n}_{iy}\mathbf{c}_{iz} & \mathbf{n}_{iy}\mathbf{n}_{ix} & \mathbf{n}_{iy}\mathbf{n}_{iy} & \mathbf{n}_{iy}\mathbf{n}_{iz}\\
%             \mathbf{n}_{iz}\mathbf{c}_{ix} & \mathbf{n}_{iz}\mathbf{c}_{iy} & \mathbf{n}_{iz}\mathbf{c}_{iz} & \mathbf{n}_{iz}\mathbf{n}_{ix} & \mathbf{n}_{iz}\mathbf{n}_{iy} & \mathbf{n}_{iz}\mathbf{n}_{iz}\\
%             \end{array}
%\right]
%\end{equation}
where $\mathbf{u}=\mathbf{v}\times \mathbf{n}$.
The covariance matrix $C$ encodes the increase of the point-to-plane error when the transformation is moved away from its optimum. The larger the error increase, the less slippable and  more stable along that transformation the shape is. On the contrary, if there is a transformation that causes small increase in the error, the shape is unstable w.r.t. the corresponding DoFs.

%By expanding $C$ in terms of its eigenvectors we may see directly the effect of various incremental transformations.
The stability can then be analyzed by calculating the eigenvalues of $C$.
Let $\lambda_1 \leq \lambda_2 \leq \cdots \leq \lambda_6$ be the eigenvalues of C.
%If some eigenvalue $\lambda_j$ is small (i.e., $\frac{\lambda_6}{\lambda_j}$ is greater than a threshold), its corresponding eigenvector (transformation) causes small error increase, meaning that the shape is unstable w.r.t the corresponding DoFs.
The stability is measured as $[1+e^{0.05\left(\frac{\lambda_6}{\lambda_1}-200\right)}]^{-1}$, where $\lambda_1$ and $\lambda_6$ are the smallest and largest eigenvalues of $C$, respectively.
%Otherwise, if no eigenvalue is small, the shape is stable under rigid transformation.
Those groups whose stability measure is greater than $0.5$ is geometrically stable.


\paragraph{Stability and object pose}
%\kx{We, for the first time, introduce the concept of stability for object pose estimation.}
Given the geometric observation of an object, we solve the problem of 6D object pose estimation on the basis of stability analysis. Specifically, we first extract a group of planar or cylindrical patches which are geometrically stable. The patches in the stable group are then aligned to the corresponding patches on the 3D model in canonical pose. Each alignment determines a subset of the six DoFs. All patches in the stable groups together pin down the 6D pose of the object. See Figure~\ref{fig:stability}(e-h) for an illustration.
In practice, however, finding patch correspondence itself is a challenging problem.
In what follows, we propose a deep neural network which predicts the 6D object pose through encoding the per-patch poses and the pair-wise patch relations.

